A Proof of $\mathfrak{L}^2$-Boundedness for Magnetic Pseudodifferential Super Operators via Matrix Representations With Respect to Parseval Frames

A fundamental result in pseudodifferential theory is the Calder\'on-Vaillancourt theorem, which states that a pseudodifferential operator defined from a H\"ormander symbol of order $0$ defines a bounded operator on $L^2(\mathbb{R}^d)$. In this work we prove an analog for pseudodifferential \emph{super} operator, \ie operators acting on other operators, in the presence of magnetic fields. More precisely, we show that magnetic pseudodifferential super operators of order $0$ define bounded operators on the space of Hilbert-Schmidt operators $\mathfrak{L}^2 \bigl ( \mathcal{B} \bigl ( L^2(\mathbb{R}^d) \bigr ) \bigr )$. Our proof is inspired by the recent work of Cornean, Helffer and Purice and rests on a characterization of magnetic pseudodifferential super operators in terms of their "matrix element" computed with respect to a Parseval frame.

==> section_6.tex <==
%!TEX root = ./humble boundedness super PsiDOs.tex
\section{Extension to operator-valued symbols} % (fold)
\label{extension_operator_valued_symbols}
%
In many applications, one encounters pseudodifferential operators defined from operator-valued functions [cite]; a recent comprehensive introduction to the topic can be found here [De Nittis, Lein \& Seri]. While we 



% section extension_to_operator_valued_symbols (end)



\section{Further applications and outlook} % (fold)
\label{outlook}
%
The utility of Gabor frames in the analysis of (magnetic) pseudodifferential \emph{super} operators seems to be as big as that for pseudodifferential operators. It stands to reason we are able to formulate and prove a commutator criterion for super operators akin to Cornean et al.\ \cite{Cornean_Helffer_Purice:simple_proof_Beals_criterion_magnetic_PsiDOs:2018} or one of the authors \cite{DeNittis_Lein_Seri:equivariant_PsiDOs:2022} did, but we will consider this question in a future work. 




% section further_applications_and_outlook (end)
